On the Complexity of Inner Product Similarity Join

A number of tasks in classification, information retrieval, recommendation systems, and record linkage reduce to the core problem of inner product similarity join (IPS join): identifying pairs of vectors in a collection that have a sufficiently large inner product. IPS join is well understood when vectors are normalized and some approximation of inner products is allowed. However, the general case where vectors may have any length appears much more challenging. Recently, new upper bounds based on asymmetric locality-sensitive hashing (ALSH) and asymmetric embeddings have emerged, but little has been known on the lower bound side. In this paper we initiate a systematic study of inner product similarity join, showing new lower and upper bounds. Our main results are: * Approximation hardness of IPS join in subquadratic time, assuming the strong exponential time hypothesis. * New upper and lower bounds for (A)LSH-based algorithms. In particular, we show that asymmetry can be avoided by relaxing the LSH definition to only consider the collision probability of distinct elements. * A new indexing method for IPS based on linear sketches, implying that our hardness results are not far from being tight. Our technical contributions include new asymmetric embeddings that may be of independent interest. At the conceptual level we strive to provide greater clarity, for example by distinguishing among signed and unsigned variants of IPS join and shedding new light on the effect of asymmetry.

==> prelims.tex <==
\subsection{Approximate MIPS}
%We let $||p||$ and $||p||_\infty$ denote the $\ell_2$ and $\ell_\infty$ norms of a vector $p\in \mathbb{R}^d$, and with $|x|$ the absolute value of the scalar $x\in \mathbb{R}$.
 


\subsection{Orthogonal Vectors Problem}
The Orthogonal Vectors Problem (OVP) is defined as follows:
\begin{definition}[OVP]
Given two sets $\P$ and $\Q$, each one containing $n$ vectors in $\{0,1\}^d$, detect if there exist vectors $p \in \P$ and $q \in \Q$ such that $p^Tq = 0$.
\end{definition}

 OVP  derives its hardness from the Strong Exponential Time Hypothesis, and the connection was proved by Williams~\cite{Williams05}.
 We remark that the conjectures are assumed to hold even against randomized algorithms~\cite{AbboudVY}.
  We will therefore assume the following plausible conjecture:
\begin{conjecture}[\cite{Williams05}]
   \label{conj:ovp}
   For all $\epsilon>0$ and (randomized) algorithms for the OVP problem, there exists $\gamma>0$ such that the running time of the algorithm, with $|\P|=|\Q|=n$ and $\gamma\log n$ dimensions, is not in $O( n^{2-\epsilon} )$.
\end{conjecture}

We recall that the conjecture does not hold for $d=\BO{\log n}$.
Indeed, it has recently been proved in~\cite{AbboudWY15} that there exists an algorithm for OVP running in $\BO{n^{2-\eps}}$, for some $\eps>0$, when $d=\BO{\log n}$.

Hence, in order to disprove OVP, an algorithm must be stronly subquadratic when $d=\gamma\log n$ for \emph{all} $\gamma$.
It is worth stating the negation of the conjecture, which is:
   ``There exists $\epsilon>0$ and an algorithm such that for all constant $\gamma$ the algorithm runs in time $O(n^{2-\epsilon})$ on instances of dimension $\gamma\log n$.''

The OVP conjecture, as usually stated, concerns the case where the two sides have equal size.
However in order to get hardness for the case where $|P|\neq|Q|$ we show that following  generalization of OVP has the same hardness as the usual OVP for all parameter values.
which doesn't yet appear to be well known in the OVP community\footnote{
   Some authors derive hardness directly from SETH, avoiding OVP, in order to get this lemma.
   TODO: citations.
}:

\begin{lemma}[Generalized OVP]\label{lem:genovp}
   Suppose there exists constants $\epsilon>0$, $\alpha>0$, $\beta>0$ and a (randomized) algorithm such that for all constant $\gamma$ the algorithm runs in time $O(n^{\alpha+\beta-\epsilon})$ on instances $|\P|=n^\alpha$, $|\Q|=n^\beta$ of dimension $\gamma\log n$.
   Then OVP is false.
\end{lemma}
\begin{proof}
   Without loss of generality, assume $\beta<\alpha$.
   Suppose we have an algorithm running in time $m^{\alpha+\beta-\epsilon}$ for some $\epsilon>0$.
   Take a normal OVP instance with $|\P|=|\Q|=n=m^\alpha$.
   Split $\P$ in chunks $\P_i$ of size $m^\beta$ and run the supposed asymmetric algorithm on all $(\P_i,\Q)$.
   This takes time $m^\alpha/m^\beta m^{\alpha+\beta-\epsilon} = m^{2\alpha-\epsilon} = n^{2-\epsilon/\alpha}$ contradicting OVP.
\end{proof}

